Specification-Guided Synthesis of Deadlock-Free Communication Protocol Refinements with Large Language Models

Ensuring behavioural correctness in communication protocols is a central challenge in distributed software systems, as subtle inconsistencies can lead to deadlocks. In such settings, protocol refinement - the safe substitution of a protocol that preserves correctness and compatibility with other components - is essential. Large language models (LLMs) have demonstrated strong capabilities in code generation and program synthesis, yet lack mechanisms to reliably produce outputs with correct behaviour. Formal specification approaches, such as multiparty session types (MPST), offer rigorous guarantees, including deadlock freedom, but provide limited support for automatically constructing protocol refinements. In this paper, we present Syntropy, a framework for synthesising protocol refinements guided by MPST specifications and LLMs. It incorporates refinement constraints directly into the generation process, ensuring the generated variants satisfy these guarantees. Our comprehensive evaluation indicates that Syntropy achieves 95.6%-99.5% validity while maintaining high syntactic correctness, and produces diverse, non-trivial refinements across multiple LLMs.

==> ams/async_subtyping.tex <==
In \MPST,  refinement of communication protocols involving multiple participants is captured by \emph{multiparty session subtyping}~\cite{???,???}. Formally, a session type $\stT$ is a 
 subtype of $\stTi$ if a process implementing $\stT$ can safely replace one implementing $\stTi$ 
 in any context while preserving \emph{deadlock-freedom} and \emph{communication safety}. 
 This notion of substitutability follows the standard variance  discipline~\cite{25inlaura}: subtyping is covariant on send actions and contravariant on receive actions. 


In asynchronous settings, subtyping may additionally permit certain actions to be reordered, reflecting asynchronous communication semantics.  
\emph{Asynchronous Multiparty Session Subtyping} (AMS)~\cite{DBLP:journals/pacmpl/GhilezanPPSY21} provides a \emph{sound} and \emph{complete} declarative characterisation of this relation,  ensuring safe replacement while excluding any unsafe extension. Furthermore, it allows two permutations: 
\begin{itemize}[leftmargin=-1pt, nosep]
\item[] {\bf R1.} an output may be anticipated before an input;  
\item[] {\bf R2.} same-direction actions may be reordered across participants.  
\end{itemize}

\fxPHerror{!!!PUT REORDERING EXAMPLE, OUR RUNNING EXAMPLE!!!}

AMS~\cite{DBLP:journals/pacmpl/GhilezanPPSY21} is defined over session trees,  a coinductive representation of session types. For a session type $\stT$, we write $\mathfrak{T}(\stT)$ for its tree representation. 
Let $\stFmt{\mathbb{T}}$ denote the class of \emph{generic} trees, among which we distinguish  
\emph{single-input} (SI) trees $\stFmt{\mathbb{V}}$, \emph{single-output} (SO) trees  $\stFmt{\mathbb{U}}$, and \emph{single-input-single-output} (SISO) trees $\stFmt{\mathbb{W}}$. 

\vspace{.3em}
\centerline{\(
\small
\begin{array}{l@{}}
\stFmt{\mathbb{T}} \bnfdef \stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}}
        \!\bnfsep\! \stFmt{{\&}_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}}  \!\bnfsep\! \stEnd
       \;\;\;
 \stFmt{\mathbb{W}} \bnfdef  \stFmt{\roleP ! \stLab \stSeq \stFmt{\mathbb{W}}} \!\bnfsep\! \stFmt{\roleP ? \stLab \stSeq \stFmt{\mathbb{W}}} \!\bnfsep\! \stEnd
 \\[.3em]
 \stFmt{\mathbb{U}} \bnfdef  \stFmt{\roleP ! \stLab \stSeq \stFmt{\mathbb{U}}} \!\bnfsep\! \stFmt{{\&}_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{U}}_i}} \!\bnfsep\! \stEnd
 \qquad \quad\;\;
  \stFmt{\mathbb{V}} \bnfdef  \stFmt{\roleP ? \stLab \stSeq \stFmt{\mathbb{V}}}  \!\bnfsep\! 
  \stFmt{{\oplus}_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{V}}_i}}   \!\bnfsep\!  \stEnd 
 \end{array}
\)}


\smallskip
Reorderings of SISO trees are defined using two classes of finite action sequences, ${\mathcal{A}}^{\roleP}$ and 
${\mathcal{B}}^{\roleP}$, parameterised by a participant $\roleP$.  
${\mathcal{A}}^{\roleP}$ contains receives from participants other than $\roleP$, while ${\mathcal{B}}^{\roleP}$ comprises receives from any participant and sends to participants other than $\roleP$. They are inductively defined as follows (where $\roleP \neq \roleQ$): 

\smallskip
\centerline{\(
{\mathcal{A}}^{\roleP} \bnfdef \stFmt{\roleQ ? \stLab} \bnfsep \stFmt{\roleQ ? \stLab}\mathbin{\!\mpFmt{.}\!}{\mathcal{A}}^{\roleP} \quad 
{\mathcal{B}}^{\roleP} \bnfdef \stFmt{\roleR ? \stLab} \bnfsep \stFmt{\roleQ ! \stLab}  \bnfsep 
\stFmt{\roleR ? \stLab}\mathbin{\!\mpFmt{.}\!}{\mathcal{B}}^{\roleP} \bnfsep
\stFmt{\roleQ ! \stLab}\mathbin{\!\mpFmt{.}\!}{\mathcal{B}}^{\roleP}
\)}

\smallskip
\noindent
The set $\emph{\text{act}}(\stFmt{\mathbb{W}})$ of actions of a SISO tree is defined as: 
$\emph{\text{act}}(\stEnd) = \emptyset$;  $\emph{\text{act}}(\stFmt{\roleP ? \stLab \stSeq \stFmt{\mathbb{W}}}) = \setenum{\stFmt{\roleP ?}} \cup 
\emph{\text{act}}(\stFmt{\mathbb{W}})$;  $\emph{\text{act}}(\stFmt{\roleP ! \stLab \stSeq \stFmt{\mathbb{W}}}) = \setenum{\stFmt{\roleP !}} \cup 
\emph{\text{act}}(\stFmt{\mathbb{W}})$. 
We then introduce \emph{refinement } for SISO trees. 

\begin{definition}[SISO Refinement]
\label{def:siso_refinement}
The  \emph{refinement relation} $\stRefinement$ for SISO trees is coinductively defined as:

\smallskip
\centerline{\(
\begin{array}{c}
\cinference[\iruleStRefA]{
\stFmt{\mathbb{W}} \stRefinement {\mathcal{A}}^{\roleP}\mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}}
& 
\emph{\text{act}}(\stFmt{\mathbb{W}}) = \emph{\text{act}}({\mathcal{A}}^{\roleP}\mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}})
}{
 \stFmt{\roleP ? \stLab} \mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W}} \stRefinement 
  {\mathcal{A}}^{\roleP}\mathbin{\!\mpFmt{.}\!} \stFmt{\roleP ? \stLab} \mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}}
}
\\[.3em]
\cinference[\iruleStRefB]{
\stFmt{\mathbb{W}} \stRefinement {\mathcal{B}}^{\roleP}\mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}}
& 
\emph{\text{act}}(\stFmt{\mathbb{W}}) = \emph{\text{act}}({\mathcal{B}}^{\roleP}\mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}})
}{
\stFmt{\roleP ! \stLab} \mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W}} \stRefinement 
  {\mathcal{B}}^{\roleP}\mathbin{\!\mpFmt{.}\!} \stFmt{\roleP ! \stLab} \mathbin{\!\mpFmt{.}\!}\stFmt{\mathbb{W'}}
}
\quad 
\cinference[\iruleStRefEnd]{}{
  \stEnd \stRefinement \stEnd
}
\\[.3em]
\cinference[\iruleStRefIn]{\stFmt{\mathbb{W}} \stRefinement \stFmt{\mathbb{W'}}
}{
 \stFmt{\roleP ? \stLab \stSeq \stFmt{\mathbb{W}}}  \stRefinement \stFmt{\roleP ? \stLab \stSeq \stFmt{\mathbb{W'}}}
}
\quad 
\cinference[\iruleStRefOut]{\stFmt{\mathbb{W}} \stRefinement \stFmt{\mathbb{W'}}
}{
 \stFmt{\roleP ! \stLab \stSeq \stFmt{\mathbb{W}}}  \stRefinement \stFmt{\roleP ! \stLab \stSeq \stFmt{\mathbb{W'}}}
}
\end{array}
\)}
\end{definition}



SISO-tree refinement captures \emph{safe permutations} of actions that do not introduce deadlocks or communication errors under asynchrony. To account for the co- and contravariance of selection and branching, SI and SO trees are derived via  the functions ${\llbracket \cdot \rrbracket}_{\text{SI}}$ and ${\llbracket \cdot \rrbracket}_{\text{SO}}$, respectively. 

\vspace{.4em}
\centerline{\(
\begin{array}{l@{}}
{\llbracket \stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}} \rrbracket}_{\text{SI}} = \setcomp{\stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{V}}_i}}}
{i \in I, \stFmt{{\mathbb{V}}_i} \in {\llbracket \stFmt{{\mathbb{T}}_i} \rrbracket}_{\text{SI}}}
\\[.3em]
{\llbracket \stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}} \rrbracket}_{\text{SO}} = \setcomp{\stFmt{\roleP ! \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{U}}_i}}}
{ i \in I, \stFmt{{\mathbb{U}}_i} \in {\llbracket \stFmt{{\mathbb{T}}_i} \rrbracket}_{\text{SO}}} \; 
{\llbracket \stEnd\rrbracket}_{\text{SO}} = \setenum{\stEnd}
\\[.3em]
{\llbracket \stFmt{{\&}_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}} \rrbracket}_{\text{SI}} = \setcomp{\stFmt{\roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{V}}_i}}}
{i \in I, \stFmt{{\mathbb{V}}_i} \in {\llbracket \stFmt{{\mathbb{T}}_i} \rrbracket}_{\text{SI}}} \; {\llbracket \stEnd\rrbracket}_{\text{SI}} = \setenum{\stEnd}
\\[.3em]
{\llbracket \stFmt{\&_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{T}}_i}} \rrbracket}_{\text{SO}} = \setcomp{\stFmt{\&_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{} \stSeq \stFmt{{\mathbb{U}}_i}}}
{ i \in I, \stFmt{{\mathbb{U}}_i} \in {\llbracket \stFmt{{\mathbb{T}}_i} \rrbracket}_{\text{SO}}}
\end{array}
\)}

\vspace{.4em}
Finally, asynchronous multiparty session subtyping reduces to decomposing session types into their SI, SO, and SISO trees and checking the corresponding refinements.

\begin{definition}[Asynchronous Subtyping]
\label{def:async_subtype}
The \emph{asynchronous subtyping relation} $\stSub$ over session types is defined as:

\smallskip
\centerline{\(
\small
\inference{
\forall \stFmt{\mathbb{U}} \in {\llbracket \mathfrak{T}(\stT) \rrbracket}_{\text{SO}}
\;\;
\forall \stFmt{\mathbb{V'}} \in {\llbracket \mathfrak{T}(\stTi) \rrbracket}_{\text{SI}}
\;\;
\exists \stFmt{\mathbb{W}} \in {\llbracket \stFmt{{\mathbb{U}}} \rrbracket}_{\text{SI}}
\;\;
\exists \stFmt{\mathbb{W'}} \in {\llbracket \stFmt{{\mathbb{V'}}} \rrbracket}_{\text{SO}}
\;\;
\stFmt{\mathbb{W}} \stRefinement  \stFmt{\mathbb{W'}}
}
{\stT \stSub \stTi}
\)}
\end{definition}


\fxPHerror{!!!TODO: PUT EXAMPLE!!!}

==> ams/session_types.tex <==
In Multiparty Session Type (\MPST) theory, \emph{local session types} (or simply \emph{session types}) describe 
the communication behaviour of an individual role (denoted by $\roleP, \roleQ, \roleFmt{s}, \rolePi, \ldots \in \roleSet$) from its local perspective.  
The syntax of session types, ranging over $\stT, \stTi, \stT[i], \ldots$, is inductively defined as follows: 

%\smallskip
\centerline{\(
\stT \bnfdef  \stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{\tyGround[i]} \stSeq \stT[i]} 
        \ \bnfsep \stFmt{{\&}_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{\tyGround[i]} \stSeq \stT[i]}  \ \bnfsep  \stRec{\stRecVar}{\stT} \ \bnfsep \ \stRecVar \ 
           \bnfsep  \stEnd
\)}

%\smallskip
\noindent
where $\tyGround$ denotes a basic value type carried as payload (\eg  integers, booleans, strings). 
For simplicity, we omit base types from the syntax in the remainder of the paper.  
The constructs $\stFmt{\oplus_{i \in I}\, \roleP ! \stChoice{\stLab[i]}{\tyGround[i]} \stSeq \stT[i]}$ and  
$\stFmt{{\&}_{i \in I}\, \roleP ? \stChoice{\stLab[i]}{\tyGround[i]} \stSeq \stT[i]}$ denote \emph{internal} and \emph{external choices}, corresponding to sending ($\stFmt{!}$) to or receiving ($\stFmt{?}$) from  role $\roleP$ a label 
$\stLab[i]$,  respectively. Here $I$ is non-empty and the labels $\stLab[i]$ are pairwise distinct. The type 
$\stEnd$ marks \emph{termination} (omitted where unambiguous), while $\stRec{\stRecVar}{\stT}$ introduces recursion  with variable $\stRecVar$. 

\fxPHerror{!!!TODO:PUT EXAMPLE OF SESSION TYPES!!!}
